Registering Explicit to Implicit: Towards High-Fidelity Garment mesh Reconstruction from Single Images

Fueled by the power of deep learning techniques and implicit shape learning, recent advances in single-image human digitalization have reached unprecedented accuracy and could recover fine-grained surface details such as garment wrinkles. However, a common problem for the implicit-based methods is that they cannot produce separated and topology-consistent mesh for each garment piece, which is crucial for the current 3D content creation pipeline. To address this issue, we proposed a novel geometry inference framework ReEF that reconstructs topology-consistent layered garment mesh by registering the explicit garment template to the whole-body implicit fields predicted from single images. Experiments demonstrate that our method notably outperforms its counterparts on single-image layered garment reconstruction and could bring high-quality digital assets for further content creation.

==> figures/fig_teaser.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=1.0\linewidth]{images/teaser3.pdf}
\vspace{-2mm}
\caption{Given a single in-the-wild image of a clothed human, \sysnameb can generate high-fidelity garment meshes through registering to the whole-body implicit fields. The appearances of the reconstructed garments are well aligned with the image input. %Moreover, due to its top logy consistent nature, the generated mesh be served as the starting point for further content creation like shape blending and resposing.
%depth map with global shape and surface details highly consistent with the input. The left-most are the input portraits, following by the estimated depth maps, meshes reconstructed from the depth maps, and the colored mesh.
\vspace{-3mm}
}
\label{fig:teaser}
\end{figure*}
